Managing target of opportunity (ToO) observations at Observatorio Astrof\'isico de Javalambre (OAJ)

The Observatorio Astrof\'isico de Javalambre (OAJ) is a Spanish astronomical ICTS (Unique Scientific and Technical Infrastructures) located in the Sierra de Javalambre in Teruel (Spain). It has been particularly conceived for carrying out large-sky multi-filter surveys. As an ICTS, the OAJ offers Open Time to the astronomical community, offering more than 25% through Legacy Surveys, Regular Programs (RP) and Director discretionary time (DDT). Regarding the RP, a new call for proposals is made public each semester accepting only proposals under the modality of Target of Opportunity (ToO). This contribution summarizes how ToOs are managed at OAJ presenting the different applications designed and implemented at the observatory to deal with them: the Proposal Preparation portal (to request observing time), the Phase2 Observing tool and the submitphase2 web service (to trigger the ToOs), the TAC Tracking portal (for telescope operators to support the observations) and the TACData portal (to publish and offer the images and their data products).

==> Makefile <==
# Example makefile to help you compile your ADASS proceedings
# but you really should read the ManuscriptInstructions.pdf or
# at least the README file.
# Authors should not need to modify the Makefile, please use the makedefs file, included here
#
# Version 7-oct-2023   Peter Teuben & Tyler Linder/Bob Seaman
#
# See also:   https://www.adass2022.ca/.... / ADASS2022.tar    @todo    for 2023
#
# P = paper_id    your proceedings paper ID code (the one with the XNN syntax, e.g., O12)
# V = version     your version # (1,2,..) since you can only upload unique files
# A = 1stauthor   your last name, e.g. Teuben
# E = email       your contact email for submission issues
# FIGS = *eps     your EPS figures

                    # put your paper_id here (with dash, not dot), e.g. P10-2
                    # or find your template on http://www.astro.umd.edu/~teuben/adass/papers/
P = $(shell ./detect_tex.py | grep -v '^%' | sed 's/.tex//g')
                    # keep incrementing this after each upload of your $(P)
V = 1
                    # First author (for Papercheck.py)
A = Teuben
                    # contact person email
E = teuben@gmail.com
		    # your EPS figures (can be blank, and must be base-named with $(P)_*.eps
FIGS = $(shell ls *.eps)

# override P,V,A,E,FIGS with a "makedefs" file, this is where authors should edit, not this Makefile!!!
-include makedefs

# Which command do you use to view the PDF? This is just for convenience.  (mac uses "open", linux "xdg-open")
# PDFOPEN = xdg-open
PDFOPEN = open

#  variables for proceeding editors (don't modify, for export, not for authors)
YEAR   = 2023
ATDIR  = ADASS$(YEAR)_author_template
FILES  = AdassChecks.py AdassConfig.py AdassIndex.py ADASS_template.tex ADASS_template.pdf \
	 Aindex.py FixUnprintable.py \
	 copyrightform.pdf example.bib example.eps \
	 Index.py manual2010.pdf ManuscriptInstructions.pdf PaperCheck.py \
	 README subjectKeywords.txt TexScanner.py \
	 ascl.py asclKeywords.txt detect_tex.py \
	 adass$(YEAR).bib Makefile makedefs \
	 $(FILESASP)

#  @todo new PID_URL ?
#  probably don't change these either (or notify the editors you have a special paper case)
PID_URL   = "https://www.canfar.net/storage/vault/list/adass2022/upload/$(P)"
TAR_FILE  = $(P).tar.gz
ZIP_FILE  = $(P).zip
POS_FILE  = $(P).pdf
FILESPDF  = $(P).pdf copyrightForm_$(P)_$(A).pdf
FILESTEX  = $(P).tex $(P).bib $(FIGS) makedefs
FILESASP  = asp2014.bst asp2014.sty
FILES4AR  = $(FILESTEX) $(FILESPDF)

# ensure current directory is in the PATH
export PATH := .:$(PATH)

help:
	@echo AUTHOR targets:
	@echo ---------------
	@echo all:   pdf check tar
	@echo pdf:
	@echo check:
	@echo clean:
	@echo overleaf:
	@echo tar:
	@echo zip:
	@echo 
	@echo EDITOR targets:
	@echo ---------------
	@echo fix:
	@echo inc:
	@echo spell:
	@echo aindex:
	@echo words:
	@echo asp1:
	@echo index:   needs TERMS=
	@echo ascl:
	@echo ascl1:
	@echo ascl2:   needs CODE=
	@echo pdf2:
	@echo rsync:


all:	pdf check tar


# not for authors, for creator of the ADASS instruction tar/zip file

aADASS_template.pdf:
	$(MAKE) P=ADASS_template

export: ADASS_template.pdf
	rm -rf $(ATDIR)
	mkdir  $(ATDIR)
	cp -a $(FILES) $(ATDIR)
	echo Created on `date` by `whoami`  > $(ATDIR)/VERSION
	-git remote -v                     >> $(ATDIR)/VERSION
	-git branch                        >> $(ATDIR)/VERSION
	-git rev-list --count HEAD         >> $(ATDIR)/VERSION
	rm -f ADASS$(YEAR).tar ADASS$(YEAR).zip
	tar cf ADASS$(YEAR).tar $(ATDIR)
	zip -urq ADASS$(YEAR).zip $(ATDIR)

# copyright is now part of the tar/zip file, checksum (sum) is 13785
copyrightForm_$(P)_$(A).pdf: copyrightform.pdf
	cp copyrightform.pdf copyrightForm_$(P)_$(A).pdf
	@echo Now go edit your copyrightForm_$(P)_$(A).pdf form

# these targets are for most common unix systems, but YMMV. Modify if you need
# let the editors know you have a better way for the next ADASS team
# ASP prefers the latex;latex;dvipdfm route

DVIPDF = dvipdf

pdf:	$(P).pdf
	@echo $(PDFOPEN) $(P).pdf 

$(P).pdf:  $(P).dvi $(FIGS)
	$(DVIPDF) $(P)

$(P).bib:                                  # bootstrap if you don't have one
	touch $(P).bib

$(P).dvi:  $(P).tex $(P).bib
	latex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	latex $(P)
	latex $(P)

# an alternative method (ASP does not recommend it)
pdflatex:
	pdflatex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	pdflatex $(P)
	pdflatex $(P)

clean:
	rm -f $(P).dvi $(P).bbl $(P).blg $(P).pdf $(P).aux $(P).log $(P).out $(P).toc $(P)_inc.tex

check:
	PaperCheck.py $(P) $(A)

ENCODING =
fix:
	FixUnprintable.py  $(P).tex $(ENCODING)

inc:
	tex2inc.py $(P).tex > $(P)_inc.tex
	@tail -1 $(P)_inc.tex
	@cat $(P).toc

spell:
	aspell --mode=tex --lang=en check $(P).tex
	@echo Share your ~/.aspell.en.pws  ~/.aspell.en.prepl

aspell:
	(cd ../..; $(MAKE) aspell)

dvi:
	latex $(P)

aindex:
	Aindex.py $(P)

DETEX = detex
words:
	$(DETEX) $(P).tex | grep -o -E '\w+' | tr '[A-Z]' '[a-z]' | sort | uniq -c | sort -n

#  could add a checksum on personal copyrightform - if it's 13785,it's bad.
tar:    $(FILES4AR) _checksum
	tar zcf $(TAR_FILE) $(FILES4AR)
	@echo "Login and upload $(TAR_FILE) at $(PID_URL)"

zip:    $(FILES4AR) _checksum
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILES4AR)
	@echo "Login and upload $(ZIP_FILE) at $(PID_URL)"

poster: $(POS_FILE)
	@echo "Login and upload $(POS_FILE) at $(PID_URL)"

overleaf:    $(FILESTEX)
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILESTEX) $(FILESASP)
	@echo You can now upload $(ZIP_FILE) as a new project into overleaf
	@echo After import, git clone this here, and move all the git tree files here.
	@echo "The git clone command is under overleaf's Menu"


_checksum: copyrightForm_$(P)_$(A).pdf
	@echo Checksum test
	@sum copyrightForm_$(P)_$(A).pdf

# for editors
asp1:
	(cd ../..; $(MAKE) asp1 PID=$(P); grep box asp1.log)
	@echo $(PDFOPEN) ../../authors/$(P).pdf

TERMS = foobar
index:
	@echo Using TERMS=$(TERMS)
	(cd ../Author_Template; Index.py $(TERMS))

ssindex:
	@echo Generating ssindex list
	(cd ../Author_Template; ssindex-org.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ssindex2:
	@echo Generating scored ssindex list 
	(cd ../Author_Template; ssindex-scored.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

index2:
	(cd ../adass_subject_recommender ; detex ../$(P)/$(P).tex |  PYTHONPATH=`pwd` bin/find_subjects.py -m 10 -j)

ascl:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)
# 	(cd ../Author_Template; ascl-new.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ascl1:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex | grep ooindex | sort | uniq -c)
	-detex $(P).tex > $(P).txt
	-(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).txt | grep ooindex | sort | uniq -c)
	-grep ooindex $(P).tex

CODE = foobar
.PHONY: ascl2
ascl2:
	$(PDFOPEN) https://ascl.net/$(CODE)

pdf2:   pdf asp1
	$(PDFOPEN) $(P).pdf
	$(PDFOPEN) ../../authors/$(P).pdf

rsync: $(P).bib
	rsync -av $(P)_inc.tex $(P).bib $(FIGS) ../../authors
	rm -f ../../authors/$(P)_inc.{bbl,blg}



==> README <==
README ADASS2024.tar
Last updated: 2024-09-20 by Peter Teuben, Tyler Linder, and Rob Seaman


Table of contents
=================

  * Introduction
  * STEP 1: Prepare your manuscript 
  * STEP 2: Check your manuscript
  * STEP 3: Package and submit your paper
  * File index
  * Github


Introduction
============

This package of files is supplied to help you prepare papers for submission in 
the Proceedings for the ADASS 2024 conference hosted by the Institute of Space
Science and Astronomy at the University of Malta. Please follow the stepwise 
instructions below carefully, because the manuscript needs to be delivered to 
ASP in print quality. The more issues are solved early on in the process, the 
more time we all save.

The instructions below are intended to guide you through the process of preparing 
and submitting your contribution. We realise it is a lot of information and some
of it is duplicated. If you need additional help, please see the list of documents
below. From "too much" to "too little" information, we provide the following 
help documents in this tar file (except for your personal template):

   1. manual2010.pdf             (ASP Instructions for Authors and Editors)
   2. ManuscriptInstructions.pdf (Guidelines for preparing an ADASS paper)
   3. README                     (This file)
   4. ADASS_template.tex         (The general ADASS template)
   5. PID.tex                    (Your personalized ADASS template for your PID, e.g. P401

At the end of this README, we also provide a file index with a short description of 
all the files present in the ADASS2024.tar file. 


STEP 1: Prepare your manuscript
===============================

The best usage is to prepare your paper in this Author_Template directory. If you
author two papers, that will work too, but preparing your tar or zip file is
much easier if you use a separate Author_Template directory for each paper.

Read the ManuscriptInstructions.pdf file. The ADASS_template.tex file gives you 
a basic template for your ADASS paper. For additional details look in the 
first section of the ASP's "Instructions for Authors and Editors" (manual2010.pdf), 
but note that this is now some years old and current requirements have changed 
slightly. In particular, ADASS papers that cite references MUST supply these 
references in a .bib BibTeX file like the example.bib file provided here.

You will need to run LaTeX on your .tex file, then run BibTeX to process the
references, and then will need to run LaTeX again up to three times to get all
the cross-references right. We recommend that you use the provided Makefile 
(see next subsection), but if you prefer building manually that should work as 
well. ASP does not use pdflatex, so try and stick to latex (we only allow EPS 
figures, not PNG or JPG; see below).

Editing your paper in overleaf (https://www.overleaf.com/) is also known to work:
simply upload (as a ZIP file is the easiest) the template, the two asp2014 files,
and optionally your BIB file and EPS figures. Don't start from scratch, or your file
will be likely named main.tex. See below if you like the "make" shortcuts.


A note about Paper IDs
----------------------

Each paper will be assigned an ID known as a PID. The PID syntax in 2024 is XNnn
where X is one of:
    - I for invited talk
    - C for contributed talk
    - P for poster
    - F for focus demo
    - B for BoF
    - T for tutorial
and NN is a two-digit number.

In this document, we will be using P401 as an example PID.

Using the provided Makefile
---------------------------

We provide a Makefile to help you build, check and package your paper in the 
correct way. To use it, you need to edit the makedefs file in this directory,
or use your personalized one.
In the makedefs file, you can define the P, V, A, E and FIGS macros, for example:

# Your proceedings PID (paper ID) code:
P = P401

# Your version # (1,2,..) since you can only upload unique files
V = 1

# Your last name, e.g. Teuben
A = Teuben

# Your contact email address for submission issues
E = teuben@gmail.com

# Your EPS figures (leave blank if you don't have any)
FIGS = P401_*.eps

Please edit the makedefs file and NOT the Makefile directly. The entries in the
makedefs file will override the ones set in the Makefile. When set correctly,
you should be able to run the following make commands:

    make pdf      : Build the PDF file (possibly twice to rid some errors)
    make check    : Check the manuscript for issues
    make tar      : Build the tar file for submission
    make all      : Do all of the above
    make overleaf : Prepare a ZIP file to bootstrap your overleaf project

For overleaf users, you can add your modified makedefs file to
complete and track the files you will modify. You can then use
https://git.overleaf.com/<MAGIC_NUMBER> to clone the repo locally, and
merge it with the other files that the ADASS editors have prepared for
you (but you should not modify).  Then you can create the ZIP or TAR
file for uploading your proceedings contribution. You can even bypass
overleaf work and do the usual git pull/push to update, which can be
useful for those who prefer to work on the desktop. But check with
your co-authors to avoid a conflict.

Adding subject index entries
----------------------------

It will help the ADASS editors if you add subject index entries for important
terms mentioned in your paper. The Index.py script can help to generate these,
and full details can be found in an appendix in ManuscriptInstructions.pdf.

In your document they should appear a commented \ssindex{} entries, e.g.

   %\ssindex{foobar}

You can also use the following word-cloud type command chain in unix:

    detex $(P).tex | grep -o -E '\w+' | sort | uniq -c | sort -n

If your "unix" doesn't have detex, use cat.

Adding ASCL index entries
-------------------------

It will help the ADASS editors if you add ASCL index entries for codes that
you are mentioning in your paper. The ascl.py script can help to generate these,
but it known to give lots of false positives. Nonetheless, you can cut and paste
the correct ones (as a latex comment) in your document, e.g.

   %\ooindex{TOPCAT, ascl:1101.010}


STEP 2: Check your manuscript
=============================

Your paper should typeset without generating any LaTeX errors or warnings. 
Overfull hbox warnings in particular need to be fixed. (In some cases underfull
hbox and vbox warnings may be tolerable.)

The 'make check' command runs a python script which looks for a number of common
problems that have been found in submitted papers. You should run it on your
paper before packaging it up for submission, and should fix any problems it 
finds. This test is a copy of a basic paper checking program that will be run 
by the ADASS editors on all submitted papers.

It is also possible to run the check manually with the PaperCheck.py script. The 
header comments in PaperCheck.py describe how to run it in detail, but essentially 
all you have to do is:

    PaperCheck.py Paper Author

where Paper is the identifier for your paper, eg O10-3 or P402-2 etc, and
Author is the surname of the first author of the paper.


STEP 3: Package and submit your paper
=====================================

You should create a .tar file with a name based on the identifier for your paper and 
including a version number, starting at 1.
e.g. example P401_v1.tar. This should contain:

  - The .tex LaTeX file
  - The .bib file defining any cited references
  - And .eps graphics files used by the paper
  - The makedefs file 
  - The resulting .pdf file for the paper, so we can see how you got it.
  - A signed copyright form.

The provided Makefile could help you to build, check and package the paper. 
Make sure that you have edited the makedefs file, where the macros P, A, E, V 
and FIGS should be defined. This makedefs file is automatically included in 
your tar/zip file.

The command to build, check, and package the manuscript is:

      make pdf check tar

If there are problems typesetting your paper, your copy of the .pdf file for
the paper will at least show the editors what you expected it to look like. If
you have already supplied a paper copy of the copyright form, you do not need
to include this. Note that electronic signatures are not acceptable - sign the
form and scan it.

(Zip files are also acceptable, using the same naming convention, e.g. P401_v1.zip.)

Submit the paper
----------------

Submit the .tar file as instructed on the ADASS 2024 web site. If you need to
submit a revised version, submit ALL the required files in a new .tar file - do
not just submit the modified files - and append a version number to the name,
e.g. P401_v2.tar. This version is defined in the V= parameter in the makedefs file.

To sum up, here is an example of the files (no sub-directories please) that the editors
like to see:

   P401.tex
   P401.bib
   P401_f1.eps
   P401_f2.eps
   makedefs
   P401.pdf

you really don't need to send us *any* other type files. Save the electrons!


File index
==========

The ADASS2024.tar package contains the following files:

README                     - this file.
Makefile                   - useful for those who like terminal commands
makedefs                   - author macros to be included by the Makefile

ManuscriptInstructions.pdf - Guidelines for preparing an ADASS paper

ADASS_template.tex         - an example template file for an ADASS 2018 paper.
example.bib                - an example BibTeX file used by ADASS_template.tex
example.eps                - an example graphics file used by ADASS_template.tex

ADASS_template.pdf         - the result of running LaTeX on ADASS_template.tex

asp2014.bst                - the required ASP bibliography style file.
asp2014.sty                - the required ASP LaTeX style file.

PaperCheck.py              - a Python script used to check an ADASS paper
Index.py                   - a Python script used to generate subject index entries
Aindex.py                  - a Python script used helping to ...
FixUnprintable.py          - a Python script used helping to ...
ascl.py                    - a python script to suggest ASCL entries
AdassChecks.py             - a Python module used by PaperCheck.py
TexScanner.py              - a Python module used by AdassChecks.py
AdassConfig.py             - a Python module used by Index.py
AdassIndex.py              - a Python module used by Index.py

subjectKeywords.txt        - set of recent subject index entries, used by Index.py
asclKeywords.txt           - list of ASCL codes for the ascl.py checker

manual2010.pdf             - The ASP "Instructions for Authors and Editors".
copyrightform.pdf          - The ASP copyright form


Github
======

Although each ADASS conference will draw its proceedings preparation package, the original github
repo from which that package is drawn, is available on https://github.com/astroumd/ADASSProceedings
Typically each year will develop the new release on a branch (e.g. "2024" for the Malta version)
and merge this back to the master for the next year team goes to work.

Authors will not need to know about that, but you may run into some editor specific comments or
commands in the Makefile or the python scripts. 

good luck!

